Higher-spin quantum and classical Schur-Weyl duality for $\mathfrak{sl}_2$

It is well-known that the commutant algebra of the $U_q(\mathfrak{sl}_2)$-action on the $n$-fold tensor product of its fundamental module is isomorphic to the Temperley-Lieb algebra TL$_n(\nu)$ with fugacity parameter $\nu = -q - q^{-1}$ (at least in the generic case, i.e., when $q$ is not a root of unity, or $n$ is small enough). Furthermore, the simple $U_q(\mathfrak{sl}_2)$-modules appearing in the direct-sum decomposition of the $n$-fold tensor product module are in one-to-one correspondence with those of the Temperley-Lieb algebra. This double-commutant property is referred to as quantum Schur-Weyl duality. In this article, we investigate such a duality in great detail. We prove that the commutant of the $U_q(\mathfrak{sl}_2)$-action on any generic type-one tensor product module is isomorphic to a diagram algebra that we call the valenced Temperley-Lieb algebra TL$_\varsigma(\nu)$. This corresponds to representations with higher spin, which results in the need of valences (or colors) in the Temperley-Lieb diagrams. We establish detailed direct-sum decompositions exhibiting this duality and find explicit bases amenable to concrete calculations, important in applications. We also include a double-commutant type property for homomorphisms between different $U_q(\mathfrak{sl}_2)$-modules, realized by valenced diagrams. The diagram calculus is reminiscent to Kauffman's recoupling theory and the graphical methods developed among others by Penrose and Frenkel \& Khovanov. The results also contain the standard quantum Schur-Weyl duality as a special case, and when specialized to $q \rightarrow 1$, imply the classical Frobenius-Schur-Weyl duality for the Lie algebra $\mathfrak{sl}_2(\mathbb{C})$ and a higher-spin version thereof.

==> QSW-bibliography.tex <==
\bibitem[AKP91]{AKP91}
H.~H.~Andersen, W.~Kexin, and P.~Polo.
\newblock Representations of quantum algebras.
\newblock {\em Invent. Math.}, 104(1):1--59, 1991.

\bibitem[ALZ15]{ALZ15}
H.~H.~Andersen, G.~I.~Lehrer and R.~B.~Zhang.
\newblock Cellularity of certain quantum endomorphism algebras. 
\newblock {\em Pacific J. Math.}, 279(1-2):11--35, 2015.
%\newblock Preprint: \href{http://arxiv.org/abs/1303.0984}{arXiv:1303.0984}, 2013.

\bibitem[Bax07]{bax}
R.~J.~Baxter.
\newblock Exactly solved models in statistical mechanics.
\newblock Originally published by Academic Press, London (1982), reprinted by Dover Publications, 2007.

\bibitem[BF91]{bf}
D.~Bernard and G.~Felder. 
\newblock Quantum group symmetries in two-dimensional lattice quantum field theory.
\newblock {\em Nucl. Phys. B}, 365(1):98--120, 1991.


\bibitem[BP14]{BP14}
A.~Borodin and L.~Petrov. 
\newblock Integrable probability: From representation theory to Macdonald processes.
\newblock {\em Probab. Surveys}, 11, 1--58, 2014.

\bibitem[BP15]{BP15}
A.~Borodin and L.~Petrov. 
\newblock Lectures on Integrable Probability: stochastic vertex models and symmetric functions.
\newblock Stochastic Processes and Random Matrices: Lecture Notes of the Les Houches Summer School: Vol. 104, July 2015.

%\bibitem[BPZ84]{bpz}
%A.~A.~Belavin, A.~M.~Polyakov, and A.~B.~Zamolodchikov.
%\newblock Infinite conformal symmetry in two-dimensional quantum field theory
%\newblock {\em Nucl. Phys. B}, 241(2):333--380, 1984.
%
%\bibitem[BR99]{br}
%H.~Barcelo and A.~Ram. 
%\newblock Combinatorial representation theory.
%\newblock In {\em New Perspectives in Geometric Combinatorics}, MSRI Publications, vol.~38, 1999.
%
%\bibitem[BSA88]{bsa}
%L.~Benoit and Y.~Saint-Aubin.
%\newblock Degenerate conformal field theories and explicit expressions for some null vectors.
%\newblock {\em Phys. Lett. B}, 215(3):517--522, 1988.
%

\bibitem[BFGT09]{BFGT09}
P.~V.~Bushlanov, B.~L.~Fe{\u\i}gin, A.~M.~Gainutdinov, and I.~Yu.~Tipunin.
\newblock Lusztig limit of quantum $\mathfrak{sl}(2)$ at root of unity and fusion of $(1,p)$ {V}irasoro logarithmic minimal models.
\newblock {\em Nucl. Phys. B}, 818(3):179--195, 2009.

\bibitem[CGRS16]{CGRS16}
G.~Carinci, C.~Giardin\`a, F.~Redig, and T.~Sasamoto. 
\newblock A generalized asymmetric exclusion process with $U_q(\mathfrak{sl}_2)$ stochastic duality. 
\newblock {\em Probab. Theory Rel. Fields}, 166(3-4):887--933, 2016.

\bibitem[CFS95]{cfs}
J.~S.~Carter, D.~E.~Flath, and M.~Saito. 
\newblock The classical and quantum $6j$-symbols.
\newblock Princeton University Press, 1995.
%
%\bibitem[CKL08]{ckl}
%G.~Chen, L.~H.~Kauffman and S.~J.~Lomonaco Jr. (editors). 
%\newblock Mathematics of quantum computation and quantum technology.
%\newblock Chapman \& Hall/CRC, 2008.
%%\newblock Chapman \& Hall/CRC Applied Mathematics and Nonlinear Science Series.
%

\bibitem[CK98]{ack}
A.~Connes and D.~Kreimer. 
\newblock Hopf Algebras, Renormalization and Noncommutative Geometry.
\newblock {\em Comm. Math. Phys.}, 199(1):203--242, 1998.


\bibitem[CP94]{cp}
V.~Chari and A.~Pressley.
\newblock A guide to quantum groups.
\newblock Cambridge University Press, 1994.

%
%\bibitem[DF84]{df1}
%V.~S.~Dotsenko and V.~A.~Fateev.
%\newblock Conformal algebra and multipoint correlation functions in $2D$ statistical models.
%\newblock {\em Nucl. Phys. B}, 240(3):312--348, 1984.
%
%\bibitem[DF85]{df2}
%V.~S.~Dotsenko and V.~A.~Fateev.
%\newblock Four-point correlation functions and the operator algebra in 2D conformal invariant theories with central charge $c\leq1$.
%\newblock {\em Nucl. Phys. B}, 251: 691--673, 1985.
%
%\bibitem[DGG97]{fgg}
%P.~Di Francesco, O.~Golinelli, and E.~Guitter. 
%\newblock Meanders and the Temperley-Lieb algebra. 
%\newblock {\em Comm. Math. Phys.}, 186(1):1--59, 1997.

%
%\bibitem[Dri87]{vd} 
%V.~G.~Drinfeld, 
%\newblock Quantum groups.
%\newblock In Proc.~ICM (Berkeley 1986).
%\newblock American Mathematical Society (Providence, RI), 798--820, 1987.

\bibitem[DJ89]{dj}
R.~Dipper and G.~James.
\newblock The $q$-Schur algebra. 
\newblock {\em Proc. London Math. Soc.}, 59(1):23--50, 1989.

%
%\bibitem[DMS97]{fms}
%P.~Di Francesco, R.~Mathieu, and D.~S\'{e}n\'{e}chal.
%\newblock Conformal field theory.
%\newblock Springer-Verlag (New York), 1997.
%
%\bibitem[Dub06]{dub}
%J.~Dub\'{e}dat.
%\newblock Euler integrals for commuting SLEs.
%\newblock {\em J. Stat. Phys.}, 123(6):1183--1218, 2006.



\bibitem[EGH{\etalchar{+}}11]{etingof}
P.~Etingof, O.~Golberg, S.~Hensel, T.~Liu, A.~Schwendner, D.~Vaintrob, and E.~Yudovina.
\newblock Introduction to representation theory.
\newblock American Mathematical Society (Providence, RI), 2011. 
%Student mathematical library, Vol~59
%\href{http://www-math.mit.edu/~etingof/replect.pdf}{http://www-math.mit.edu/~etingof/replect.pdf}.

\bibitem[Fel89]{Felder}
G.~Felder.
\newblock B{RST} approach to minimal models.
\newblock {\em Nucl. Phys. B}, 317(1):215--236, 1989.
\newblock Erratum ibid. B, 324(2):548, 1989.

%\bibitem[FFK89]{ffk}
%G.~Felder, J.~Fr{\"o}hlich, and G.~Keller.
%\newblock Braid matrices and structure constants for minimal conformal models.
%\newblock {\em Comm. Math. Phys.}, 124(4):647--664, 1989.

\bibitem[FK97]{fk}
I.~B.~Frenkel and M.~G.~Khovanov.
\newblock Canonical bases in tensor products and graphical calculus for $U_q(\mathfrak{sl}_2)$.
\newblock {\em Duke Math. J.}, 87(3):409--480, 1997.

\bibitem[FKK98]{fkk}
I.~Frenkel, M.~Khovanov, and A.~Kirillov~Jr.
\newblock Kazhdan-Lusztig polynomials and canonical basis.
\newblock {\em Transform. Groups}, 3(4):321--336, 1998.

%\bibitem[FK15a]{sfk1}
%S.~M.~Flores and P.~Kleban.
%\newblock A solution space for a system of null-state partial differential equations 1.
%\newblock {\em Comm. Math. Phys.}, 333(1):389--434, 2015.
%
%\bibitem[FK15b]{sfk2}
%S.~M.~Flores and P.~Kleban.
%\newblock A solution space for a system of null-state partial differential equations 2.
%\newblock {\em Comm. Math. Phys.}, 333(1):435--481, 2015.
%
%\bibitem[FK15c]{sfk3}
%S.~M.~Flores and P.~Kleban.
%\newblock A solution space for a system of null-state partial differential equations 3.
%\newblock {\em Comm. Math. Phys.}, 333(2):597--667, 2015.
%
%\bibitem[FK15d]{sfk4}
%S.~M.~Flores and P.~Kleban
%\newblock A solution space for a system of null-state partial differential equations 4.
%\newblock {\em Comm. Math. Phys.}, 333(2):669--715, 2015.


\bibitem[FKS06]{fks}
I.~Frenkel, M.~Khovanov, and C.~Stroppel.
\newblock A categorification of finite-dimensional irreducible representations of quantum $\mathsf{U}_q\mathfrak{sl}(2)$ and their tensor products. 
\newblock {\em Selecta Math. (N.S.)}, 12(3-4):379--431, 2006.

\bibitem[FP18a]{fp3a}
S.~M.~Flores and E.~Peltola. 
\newblock Standard modules, radicals, and the valenced Temperley-Lieb algebra.
\newblock Preprint: \href{http://arxiv.org/abs/1801.10003}{arXiv:1801.10003}, 2018.

\bibitem[FP18b]{fp3b}
S.~M.~Flores and E.~Peltola. 
\newblock Generators, projectors, and the Jones-Wenzl algebra. 
\newblock Preprint: \href{http://arxiv.org/abs/1811.12364}{arXiv:1811.12364}, 2018.

\bibitem[FP20a{\etalchar{+}}]{fp2}
S.~M.~Flores and E.~Peltola. 
\newblock Solution spaces of the Benoit \& Saint-Aubin partial differential equations.
\newblock  In preparation.

\bibitem[FP20b{\etalchar{+}}]{fp1}
S.~M.~Flores and E.~Peltola. 
\newblock Monodromy invariant CFT correlation functions of first column Kac operators.
\newblock  In preparation.


%\bibitem[FSK15]{fsk}
%S.~M.~Flores, J.~J.~H.~Simmons, and P.~Kleban.
%\newblock Multiple-SLE$_\kappa$ connectivity weights for rectangles, hexagons, and octagons.
%\newblock Preprint: \href{http://arxiv.org/abs/1505.07756}{arXiv:1505.07756}, 2015.
%
%\bibitem[FSS12]{fss}
%I.~Frenkel, C.~Stroppel, and J.~Sussan.
%\newblock Categorifying fractional Euler characteristics, Jones-Wenzl projector and $3j$-symbols.
%\newblock {\em Quantum Topol.}, 3(2):181--253, 2012.
%
%\bibitem[Fuc92]{fuc}
%J.~Fuchs. 
%\newblock Affine Lie algebras and quantum groups.
%%\newblock Cambridge Monographs on Mathematical Physics.
%\newblock Cambridge University Press, 1992. 
%
%\bibitem[FW91]{fw}
%G.~Felder and C.~Wieczerkowski.
%\newblock Topological representations of the quantum group $U_q(\mathfrak{sl}_2)$.
%\newblock {\em Comm. Math. Phys.}, 138(3):583--605, 1991. 


\bibitem[GST14]{GST14}
A.~M.~Gainutdinov, H.~Saleur, and I.~Yu.~Tipunin.
\newblock Lattice {W}-algebras and logarithmic {CFT}s.
\newblock {\em J. Phys.~A: Math. Theor.}, 47(49):495401, 2014.


\bibitem[GL96]{gl}
J.~J.~Graham and G.~I.~Lehrer.
\newblock Cellular algebras.
\newblock {\em Invent. Math.}, 123(1):1--34, 1996.

\bibitem[GL98]{gl2}
J.~J.~Graham and G.~I.~Lehrer.
\newblock The representation theory of affine Temperley-Lieb algebras. 
\newblock {\em Enseign. Math.}, 44(3-4):173--218, 1998.

\bibitem[GRAS96]{gras}
C.~G{\'o}mez, M.~Ruiz-Altaba, and G.~Sierra.
\newblock Quantum groups in two-dimensional physics.
\newblock Cambridge University Press, 1996.

%\bibitem[GS90]{gs}
%C.~G{\'o}mez and G.~Sierra.
%\newblock Quantum group meaning of the Coulomb gas.
%\newblock {\em Phys. Lett. B}, 240(1-2):149--157, 1990.
%
%\bibitem[Gre07]{jag}
%J.~A.~Green.
%\newblock Polynomial representations of $GL_n$.
%\newblock Springer-Verlag Berlin Heidelberg, 2nd Ed., 2007.
%%Lecture Notes in Mathematics, Vol. 830

\bibitem[GV13]{gv}
A.~M. Gainutdinov and R.~Vasseur.
\newblock Lattice fusion rules and logarithmic operator product expansions.
\newblock {\em Nucl. Phys. B}, 868(1):223--270, 2013.

\bibitem[GW93]{gwe}
F.~M.~Goodman and H.~Wenzl.
\newblock The Temperley-Lieb algebra at roots of unity. 
\newblock {\em Pacific J. Math.}, 161(2):307--334, 1993.

%\bibitem[GW98]{gw}
%R.~Goodman and N.~R.~Wallach.
%\newblock Representations and invariants of the classical groups.
%\newblock Cambridge University Press, 1998.

\bibitem[GW09]{gw2}
R.~Goodman and N.~R.~Wallach.
\newblock Symmetry, representations, and invariants. 
%\newblock Graduate Texts in Mathematics, vol. 255.
\newblock Springer (Dordrecht Heidelberg London New York), 2009.

%
%\bibitem[Hen99]{mh}
%M.~Henkel. 
%\newblock Conformal invariance and critical phenomena.
%\newblock Springer-Verlag (Berlin Heidelberg), 1999.
%
%\bibitem[ILZ19]{ilz}
%K.~Iohara, G.~I.~Lehrer, and R.~B.~Zhang.
%\newblock Temperley-Lieb at roots of unity, a fusion category, and the Jones quotient.
%\newblock {\em Math. Res. Lett.}, 26(1):121--158, 2019.  
%

\bibitem[IWWZ13]{IWWZ}
Y.~Ikhlef, R.~Weston, M.~Wheeler, and P.~Zinn-Justin. 
\newblock Discrete holomorphicity and quantized affine algebras.
\newblock {\em J. Phys. A}, 46(26): 265205, 2013.

%\bibitem[JM79]{jm79}
%G.~James and G.~Murphy.
%\newblock The determinant of the Gram matrix for a Specht module.
%\newblock {\em J. Alg.}, 59(1):222--235, 1979.
%
%\bibitem[Jim85]{mj1}
%M.~Jimbo. 
%\newblock A $q$-difference analog of $U(\mathfrak{g})$ and the Yang-Baxter equation.
%\newblock {\em Lett. Math. Phys.}, 1(10):63--69, 1985.
%% Eve: this reference defined the quantum groups for general Lie algebras $\mathfrak{g}$.
%% In the case of $\mathfrak{g} = \mathfrak{sl}_2$, $U_q(\mathfrak{sl}_2)$ was introduced by Kulish and Reshetikin in~\cite{kr}

\bibitem[Jim86]{mj2}
M.~Jimbo.
\newblock A $q$ analog of $\mathcal{U}(\mathfrak{gl}(N+1))$, Hecke algebra, and the Yang-Baxter equation.
\newblock {\em Lett. Math. Phys.}, 3(11):247--252, 1986. 

\bibitem[JJK16]{jjk}
N.~Jokela, M.~J{\"a}rvinen, and K.~Kyt{\"o}l{\"a}.
\newblock SLE boundary visits.
\newblock {\em Ann. Henri Poincar\'e}, 17(6):1263--1330, 2016.

\bibitem[Jon83]{vj}
V.~F.~R.~Jones.
\newblock Index for subfactors. 
\newblock {\em Invent. Math.}, 72(1):1--25, 1983.

%\bibitem[Jon86]{vj3}
%V.~F.~R.~Jones.
%\newblock Braid groups, Hecke algebras, and type $II_1$ factors.
%\newblock In {\em Geometric Methods in Operator Algebras, Proc. US-Japan Seminar (Kyoto 1983)},
%Pitman Res. Notes Math. Ser., 123:242--273, 1986.
%
%\bibitem[Jon89]{vj2}
%V.~F.~R.~Jones.
%\newblock On knot invariants related to some statistical mechanical models. 
%\newblock {\em Pacific J. Math.}, 137(2):311--334, 1989.

\bibitem[Kas95]{ck}
C.~Kassel.
\newblock Quantum groups.
%\newblock Graduate Texts in Mathematics. 
\newblock Springer-Verlag (New York), 1995.

%\bibitem[Kau87]{lk2}
%L.~H.~Kauffman.
%\newblock State models and the Jones polynomial.
%\newblock {\em Topology}, 26(3):395--407, 1987. 

\bibitem[Kau90]{lk}
L.~H.~Kauffman.
\newblock An invariant of regular isotopy.
\newblock {\em Trans. Amer. Math. Soc.}, 318(2):417--471, 1990. 


\bibitem[KKP19]{kkp}
A.~Karrila, K.~Kyt\"ol\"a, and E.~Peltola.
\newblock Conformal blocks, $q$-combinatorics, and quantum group symmetry.
\newblock {\em Ann. Inst. Henri Poincar{\'e} D}, 6(3):449--487, 2019.

\bibitem[KL94]{kl}
L.~H.~Kauffman and S.~L.~Lins. 
\newblock Temperley-Lieb recoupling theory and invariants of $3$-manifolds.
\newblock Princeton University Press, 1994.

%\bibitem[KM13]{km}
%N.-G.~Kang and N.~Makarov. 
%\newblock Gaussian free field and conformal field theory.
%\newblock {\em Ast\'erisque}, 353, 2013.

\bibitem[KR81]{kr}
P.~P.~Kulish and N.~Yu~Reshetikhin. 
\newblock Quantum linear problem for the sine-Gordon equation and higher representations.
\newblock {\em Zap. Nauchn. Sem. Leningrad. Otdel. Mat. Inst. Steklov. (LOMI)}, 101:101-110, 1981.
\newblock Transl. {\em J.~Soviet Math.}, 23(4):2435--2441, 1983. 

\bibitem[KP16]{kp}
K.~Kyt\"ol\"a and E.~Peltola.
\newblock Pure partition functions of multiple SLEs.
\newblock {\em Comm. Math. Phys.}, 346(1):237--292, 2016.

\bibitem[KP19]{kp2}
K.~Kyt\"ol\"a and E.~Peltola.
\newblock Conformally covariant boundary correlation functions with a quantum group.
\newblock \emph{J.~Eur. Math. Soc}, to appear, 2020.
\newblock Preprint: \href{http://arxiv.org/abs/1408.1384}{arXiv:1408.1384}.

\bibitem[KRT97]{krt}
C.~Kassel, M.~Rosso, and V.~G.~Turaev.
\newblock Quantum groups and knot invariants.
\newblock American Mathematical Society, 1997. 

%\bibitem[KS97]{ks}
%A.~Klimyk and K.~Schm\"udgen. 
%\newblock Quantum Groups and Their Representations. 
%\newblock Springer-Verlag Berlin Heidelberg, 1997.

\bibitem[KMMO16]{KMMO16}
A.~Kuniba, V.~Mangazeev, S.~Maruyama, M.~Okado 
\newblock Stochastic R-Matrix for $U_Q(A_N^{(1)})$.
\newblock {\em Nucl. Phys. B}, 913:248--277, 2016.


\bibitem[Lam91]{lam}
T.~Y.~Lam. 
\newblock A first course in non-commutative rings.
%\newblock Graduate Texts in Mathematics. 
\newblock Springer-Verlag (Berlin Heidelberg), 1991.

%\bibitem[LS90]{ls}
%S.~Z.~Levendorskii and Ya.~S.~Soibelman.
%\newblock Some applications of quantum Weyl groups.
%\newblock {\em J.~Geom.~Phys.}, 7(2):241--254, 1990.

\bibitem[Lus89]{Lus89}
G.~Lusztig.
\newblock Modular representations and quantum groups.
\newblock {\em Contemp. Math.}, 82:59--77, 1989.

%\bibitem[Lus90a]{Lus90} %{glu}
%G.~Lusztig.
%\newblock On quantum groups.
%\newblock {\em J.~Algebra}, 131(2):466--475, 1990.

\bibitem[Lus90]{Lusz}
G.~Lusztig.
\newblock Finite-dimensional Hopf algebras arising from quantized universal enveloping algebra. .
\newblock {\em J. Amer. Math. Soc.}, 3:257--296, 1990.

\bibitem[Man18]{man}
Y.~I.~Manin. 
\newblock Quantum Groups and Noncommutative Geometry
\newblock Springer Nature Switzerland AG, 2nd Edition, 2018.

\bibitem[Mar91]{pm}
P.~P.~Martin. 
\newblock Potts models and related problems in statistical mechanics.
\newblock World Scientific (Singapore), 1991.

\bibitem[Mar92]{ppm}
P.~P.~Martin. 
\newblock On Schur-Weyl duality, $A_n$ Hecke algebras and quantum $\mathfrak{sl}(N)$ on $\otimes^{n+1} \bC^N$.
\newblock {\em Int. J. Mod. Phys. A}, 7: Supp.~1B, 645--673, 1992.

\bibitem[Mat99]{am}
A.~Mathas. 
\newblock Iwahori-Hecke algebras and Schur algebras of the symmetric group.
\newblock University Lecture Series, Vol.~15.
\newblock American Mathematical Society (Providence RI) 1999.

\bibitem[MDRR15]{mrr}
A.~Morin-Duchesne, J.~Rasmussen, and D.~Ridout.
\newblock Boundary algebras and Kac modules for logarithmic minimal models.
\newblock {\em Nucl. Phys. B}, 889:677--769, 2015.

\bibitem[MMA92]{mma}
P.~P.~Martin and D.~McAnally.
\newblock On commutants, dual pairs and non-semisimple algebras from statistical mechanics.
\newblock {\em Int. J. Mod. Phys. A}, 7: Supp.~1B, 675--705, 1992.

%
%\bibitem[Mor15]{sm}
%S.~Morrison.
%\newblock A formula for the Jones-Wenzl projections.
%\newblock Preprint: \href{http://arxiv.org/abs/1503.00384}{arXiv:1503.00384}, 2015.

\bibitem[MR89]{mr}
G.~Moore and N.~Yu.~Reshetikhin. 
\newblock A comment on quantum group symmetry in conformal field theory.
\newblock {\em Nucl. Phys. B}, 328(3):557--574, 1989.

\bibitem[MV94]{mv}
G.~Masbaum and P.~Vogel.
\newblock $3$-valent graphs and the Kauffman bracket. 
\newblock {\em Pacific J. Math.}, 164(2):361--381, 1994.

\bibitem[PS90]{ps}
V.~Pasquier and H.~Saleur.
\newblock Common structures between finite systems and conformal field theories through quantum groups. 
\newblock {\em Nucl. Phys. B}, 330(2-3):523--556, 1990.

\bibitem[Pel20]{ep2} 
E.~Peltola.
\newblock Basis for solutions of the Benoit \& Saint-Aubin PDEs with particular asymptotic properties.
\newblock \emph{Ann. Inst. Henri Poincar\'e D,} to appear, 2020.
\newblock Preprint: \href{http://arxiv.org/abs/1605.06053}{arXiv:1605.06053}. 

\bibitem[Pen71]{pen}
R.~Penrose.
\newblock Angular momentum: an approach to combinatorial space-time.
\newblock In {\em Quantum Theory and Beyond} (T.~Bastin ed.), Cambridge University Press, pp. 151--180, 1971. 

%\bibitem[Pie82]{rp}
%R.~S.~Pierce.
%\newblock Associative algebras.
%\newblock Springer-Verlag (NewYork Heidelberg Berlin), 1982.
%

\bibitem[PSA14]{psa}
G.~Provencher and Y.~Saint-Aubin.
\newblock The idempotents of the $\mathrm{TL}_n$-module $\otimes^n\mathbb{C}2$ in terms of elements of $\mathcal{U}_q(\mathfrak{sl}_2)$.
\newblock {\em Ann. Henri Poincar\'e}, 15(11):2203--2240, 2014.

%\bibitem[RS07a]{rs1}
%N.~Read and H.~Saleur.
%\newblock Enlarged symmetry algebras of spin chains, loop models, and {S}-matrices. 
%\newblock {\em Nucl. Phys. B}, 777(3):263--315, 2007.

%\bibitem[RS07b]{rs2}
\bibitem[RS07]{rs2}
N.~Read and H.~Saleur.
\newblock Associative-algebraic approach to logarithmic conformal field theories.
\newblock {\em Nucl. Phys. B}, 777(3):316--351, 2007.

\bibitem[RT91]{rt}
N.~Yu.~Reshetikhin and V.~G.~Turaev. 
\newblock Invariants of three manifolds via link polynomials and quantum groups. 
\newblock {\em Invent. Math.}, 103:547--597, 1991.

%\bibitem[Rib14]{sr}
%S.~Ribault.
%\newblock Conformal field theory on the plane.
%\newblock Preprint: \href{http://arxiv.org/abs/1406.4290}{arXiv:1406.4290}, 2014.

\bibitem[RSA14]{rsa}
D.~Ridout and Y.~Saint-Aubin.
\newblock Standard modules, induction, and the structure of the Temperley-Lieb algebra.
\newblock {\em Adv. Theor. Math. Phys.}, 18(5):957--1041, 2014.

\bibitem[RTW32]{rtw}
G.~Rumer, E.~Teller, and H.~Weyl.
\newblock Eine f\"ur die Valenztheorie geeignete Basis der bin\"aren Vektorinvarianten. 
\newblock Nachrichten von der Ges. der Wiss. Zu Go\"ottingen. Math.-Phys. Klasse, 498--504, 1932

%
%\bibitem[Sch08]{sch}
%M.~Schottenloher.
%\newblock A mathematical introduction to conformal field theory.
%\newblock Springer-Verlag (Berlin Heidelberg), 2008.

\bibitem[Sch27]{schur}
I.~Schur.
\newblock \"Uber die rationalen Darstellungen der allgemeinen linearen Gruppe.
\newblock Sitzungsberichte Akad. Berlin, 58--75, 1927

\bibitem[Sha05]{irs}
I.~R.~Shafarevich.
\newblock Basic notions of algebra.
\newblock Springer-Verlag (Berlin Heidelberg), 2005.

%
%\bibitem[SS14]{ss}
%C.~Stroppel and J.~Sussan. 
%\newblock Categorified Jones-Wenzl projectors: a comparison.
%\newblock In {\em Perspectives in representation theory, Contemp. Math.}, vol.~610.
%\newblock American Mathematical Society (Providence RI), 333--351, 2014.

\bibitem[Str10]{cs}
C.~Stroppel.
\newblock Schur-Weyl dualities and link homologies.
\newblock In {\em Proc. ICM 2010, Hyderabad, India}, 2010.


\bibitem[TL71]{tl}
H.~Temperley and E.~Lieb. 
\newblock Relations between the `percolation' and `colouring' problem 
and other graph-theoretical problems associated with regular planar lattices: some exact results for the `percolation' problem.
\newblock In {\em Proc. Roy. Soc. London Ser. A}, 322:251--280, 1971. 

\bibitem[Tur94]{vt}
V.~G.~Turaev.
\newblock Quantum invariants of knots and $3$-manifolds.
\newblock Walter de Gruyter (Berlin New York) 1994. 


\bibitem[Var92]{var}
A.~Varchenko.
\newblock Multidimensional hypergeometric functions in conformal field theory,
  algebraic {K-theory}, algebraic geometry.
\newblock In {\em Proceedings of the {International} {Congress} of
  {Mathematicians}, Kyoto 1990}, 1992.
  
\bibitem[Wan10]{zw}
Z.~Wang.
\newblock Topological quantum computation.
\newblock Lecture notes, Microsoft Research, 2010.
\newblock Available at \href{http://web.math.ucsb.edu/~zhenghwa/data/course/cbms.pdf}{http://web.math.ucsb.edu/~zhenghwa/data/course/cbms.pdf}.

\bibitem[Wen87]{hw}
H.~Wenzl.
\newblock On sequences of projections.
\newblock {\em C. R. Math. Rep. Acad. Sci. Canada}, 9(1):5--9, 1987.
%
%\bibitem[Wes95]{bw}
%B.~Westbury.
%\newblock The representation theory of the Temperley-Lieb algebras.
%\newblock {\em Math. Zeit.}, 219(1):539--565, 1995.
%

\bibitem[Wey39]{hew}
H.~Weyl.
\newblock The Classical Groups. Their Invariants and Representations.
\newblock Princeton University Press, 1939.

\bibitem[Wit89]{wit}
E.~Witten. 
\newblock Quantum Field Theory and the Jones Polynomial. 
\newblock {\em Comm. Math. Phys.}, 121:351--399, 1989.

%\bibitem[Zin07]{zin}
%P. Zinn-Justin. 
%\newblock Combinatorial Point for Fused Loop Models. 
%\newblock {\em Comm. Math. Phys.}, 272(3):661--682, 2007.

==> QSchurWeyl_macros.tex <==
%EP (date July 19 2020): moved these two macros here: hey are vey useful!
\newcommand{\EndAlg}[2]{\smash{#1\;\scalebox{1}{\rotatebox[origin=c]{270}{$\circlearrowleft$}} \, \subscr{#2}}}
\newcommand{\Module}[2]{\smash{\superscr{#2 \;} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; #1}}

%EP (date July 19 2020): added these four macros:
%I think we should omit the macro \SpinChain etc, this is too confusing
\newcommand{\RModule}[2]{\smash{#1 \; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, \superscr{\; #2}}}
\newcommand{\CModule}[2]{\smash{\subscr{#2 \;}\scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; #1}}
\newcommand{\BIModule}[3]{\smash{\subscr{#3 \;}\superscr{#2 \;} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; #1}}
\newcommand{\BIRModule}[3]{\smash{#1 \; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, \superscr{\; #2}\subscr{\; #3}}}
%EP (date July 29 2020): one more:
\newcommand{\CRModule}[2]{\smash{#1 \; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, \subscr{\; #2}}}


%EP (date June 24 2020): 
%Note that I have inserted space "\," to all macros that involve 
%\circlearrowleft
%and 
%\circlearrowright

%EP (date June 24 2020): added: (probably become redundant)
\newcommand{\row}{\mathsf{Row}}
\newcommand{\col}{\mathsf{Col}}


%EP (date July 18 2020): added: 
\newcommand{\alg}{\mathsf{A}}
\newcommand{\almostId}{i}

%EP (date July 22 2020): added: 
\newcommand{\ProjM}{\mathsf{P}}

%EP (date July 28 2020): added: 
\newcommand{\algB}{\mathsf{A}}%{\mathsf{A}}
%NB: there are many problems with notation \mathsf{B} both with dual bases and orthogonal bases

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% SF: What is \overbarcal? I'm not using it anywhere.

%EP: 
%the positioning of the bar didn't look correct for greek letters. Therfore I use \overbarcal. E.g. \alphaBar = \overbarcal{\alpha} 

%On the other hand, \overbarStraight is better for e.g. \mathsf letters and vectors like \overbarStraight{v} and \overbarStraight{w}.

%I have removed \overbar because this way I could check that the correct shaped "bar" is used in our files.
%\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}


%now these are the same that are used in the diagram algebra papers:
\newcommand{\overbarStraight}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\overbarcal}[1]{\mkern 2.50mu\overline{\mkern-2.50mu#1\mkern-0.5mu}\mkern 0.5mu}
\newcommand{\overbarcalcal}[1]{\mkern 7.50mu\overline{\mkern-7.50mu#1\mkern-0.5mu}\mkern 0.5mu}
\newcommand{\overhat}[1]{\hstretch{1.75}{\hat{\hstretch{.57}{#1}}}}
\newcommand{\overhatcal}[1]{\mkern 2.50mu\overhat{\mkern-2.50mu#1\mkern-0.5mu}\mkern 0.5mu}
\newcommand{\overtildecal}[1]{\mkern 2.50mu\widetilde{\mkern-2.50mu#1\mkern-0.5mu}\mkern 0.5mu}


\newcommand{\alphaBar}{\overbarcal{\alpha}}
\newcommand{\betaBar}{\overbarcal{\beta}}

\newcommand{\DeltaBar}{\overbarcal{\Delta}}

\newcommand{\EBar}{\overbarcal{E}}
\newcommand{\FBar}{\overbarcal{F}}
\newcommand{\KBar}{\overbarcal{K}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\global\long\def\ud{\mathrm{d}}

\global\long\def\bR{\mathbb{R}}
\global\long\def\bRpos{\mathbb{R}_{> 0}}
\global\long\def\bRnn{\mathbb{R}_{\geq 0}}
\global\long\def\bZ{\mathbb{Z}}
\global\long\def\bN{\mathbb{N}}
\global\long\def\bZpos{\mathbb{Z}_{>0}}
\global\long\def\bZneg{\mathbb{Z}_{<0}}
\global\long\def\bZnn{\mathbb{Z}_{\geq 0}}
\global\long\def\bQ{\mathbb{Q}}
\global\long\def\bC{\mathbb{C}}
\global\long\def\tieOp{\wp}

\global\long\def\ii{\mathfrak{i}}

\global\long\def\sF{\mathcal{F}}
\global\long\def\SurfFW{\mathfrak{L}^{\Supset}}
\newcommand{\sH}{\mathcal{H}}

\newcommand{\re}{\mathfrak{Re}}

\global\long\def\pder#1{\frac{\partial}{\partial#1}}
\global\long\def\der#1{\frac{\ud}{\ud#1}}
\global\long\def\pder#1{\frac{\partial}{\partial#1}}
\global\long\def\pdder#1{\frac{\partial^{2}}{\partial#1^{2}}}
\global\long\def\pddder#1{\frac{\partial^{3}}{\partial#1^{3}}}





\newcommand{\TangleEmb}[2]{(\mathfrak{E}_{#1} \otimes \mathfrak{E}_{#2})}
\newcommand{\rad}{\textnormal{rad}\,}
\newcommand{\Span}{\textnormal{span}\,}
\newcommand{\sleg}[1]{b_{#1}}
\newcommand{\Mob}{\mu}
\newcommand{\conf}{\varphi}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\AllDefects}{\mathbin{\rotatebox[origin=c]{-90}{$\exists$}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%EP (date July 18 2020): trying out these:
\newcommand{\EndMod}[1]{\textnormal{End}_{\,#1}}
\newcommand{\EndModOp}[1]{\textnormal{End}\superscr{\textnormal{op}}_{\,#1}}

\newcommand{\HomMod}[1]{\textnormal{Hom}_{\,#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\End}{\textnormal{End}\,}
\newcommand{\Lin}{\textnormal{Lin}\,}
\newcommand{\EndOp}{\textnormal{End}\superscr{\textnormal{op}}\,}
%\newcommand{\EndMod}[2]{\textnormal{End}_{\,#1}  #2}
%\newcommand{\EndModOp}[2]{\textnormal{End}\superscr{\textnormal{op}}_{\,#1}  #2}

%\newcommand{\Aut}{\textnormal{Aut}\,}

\newcommand{\Hom}{\textnormal{Hom}\,}
%\newcommand{\Hom}{\textnormal{Lin}\,}
%\newcommand{\Hom}[2]{\textnormal{Hom}\left(#1,#2\right)}
%\newcommand{\HomOp}[2]{\textnormal{Hom}\superscr{\textnormal{op}}\left(#1,#2\right)}
%\newcommand{\HomMod}[3]{\textnormal{Hom}_{\,#1} \hspace{-1mm} \left(#2,#3\right)}
%\newcommand{\HomModOp}[3]{\textnormal{Hom}\superscr{\textnormal{op}}_{\,#1} \hspace{-1mm} \left(#2,#3\right)}
%\newcommand{\HomModMod}[2]{\textnormal{Hom}\left(#1,#2\right)}

\newcommand{\Br}{\mathsf{Br}}
\newcommand{\LS}{\mathsf{L}}
\newcommand{\LSBar}{\overbarStraight{\LS}}
\newcommand{\LSPerp}{\LS\superscr{\perp} }
\newcommand{\LSPerpBar}{\LSBar\superscr{\perp}}

\newcommand{\PairMod}[3]{#1\xrightarrow[\hspace{1.2cm}]{#2} #3}

\newcommand{\OldLeftPairMod}[3]{#1\xrightarrow[\hspace{1.2cm}]{#2} #3}
\newcommand{\OldRightPairMod}[3]{#1\xleftarrow[\hspace{1.2cm}]{#2} #3}

\newcommand{\hookuparrow}{\mathrel{\rotatebox[origin=c]{90}{$\hookrightarrow$}}}
\newcommand{\hookdownarrow}{\mathrel{\rotatebox[origin=c]{-90}{$\hookrightarrow$}}}

\newcommand{\LeftPairMod}[3]{{}^{#2\hspace{-0.1cm}}_{#3}\hookdownarrow{#1}}
\newcommand{\RightPairMod}[3]{{#1}\hspace{0.05cm}\text{\reflectbox{$\hookdownarrow$}\hspace{0.1cm}}^{#2}_{#3}}




\newcommand{\preLS}{\mathsf{pre}\,\text{-}\,\mathsf{L}}
\newcommand{\Gen}{U}
\newcommand{\ValGen}{U}%{U\super{\multii}}
\newcommand{\Lgen}{L}
\newcommand{\Rgen}{R}
\newcommand{\hatotimes}{\,\hat{\otimes}\,}
\newcommand{\Sym}{\mathfrak{S}}
\newcommand{\Quo}{\mathsf{Q}}
\newcommand{\QuoBar}{\overbarStraight{\Quo}}

\newcommand{\LP}{\mathsf{LP}}
\newcommand{\LPBar}{\overbarStraight{\LP}}

\newcommand{\preLP}{\mathsf{pre}\,\text{-}\,\mathsf{LP}}
\newcommand{\LD}{\mathsf{LD}}
\newcommand{\LDBar}{\overbarStraight{\LD}}

\newcommand{\preLD}{\mathsf{pre}\,\text{-}\,\mathsf{LD}}
\newcommand{\Lmap}{\mathcal{L}}
\newcommand{\LmapBar}{\overbarcal{\Lmap}}

\newcommand{\ThetaNet}{\Theta}%{\theta}

\newcommand{\TetraNet}{\textnormal{Tet}}%{\theta}


\newcommand{\Jones}{J}
\newcommand{\smin}{s_{\textnormal{min}}}
\newcommand{\smax}{s_{\textnormal{max}}}
\newcommand{\pmin}{\mathfrak{p}}

%\newcommand{\ppmin}{\bar{\pmin}}
\newcommand{\ppmin}{\hat{\pmin}}

\newcommand{\TL}{\mathsf{TL}}
\newcommand{\preTL}{\mathsf{pre}\,\text{-}\mathsf{TL}}
%\newcommand{\WJ}{\mathsf{WJ}}
\newcommand{\WJ}{\mathsf{JW}}
%\newcommand{\PS}{\LinkEmb\LS}

\newcommand{\PS}{\mathsf{K}}
\newcommand{\PP}{\PS\mathsf{P}}
\newcommand{\PD}{\PD\mathsf{D}}


%\newcommand{\Walks}{\mathscr{W}}

%\newcommand{\PH}{\mathsf{N}}
\newcommand{\Wd}{\mathsf{M}}
\newcommand{\WdBar}{\overbarStraight{\Wd}}


\newcommand{\Dom}{\mathsf{Non}}
\newcommand{\Tot}{\mathsf{Tot}}

\newcommand{\MTbas}{\theta}
\newcommand{\MTbasBar}{\overbarcal{\MTbas}}

\newcommand{\mult}{\text{mult}}
%\newcommand{\sing}{\mathcalligra{s}}
\newcommand{\sing}{\mathcalligra{s}\,}
\newcommand{\singBar}{\overbarcal{\sing}}

\newcommand{\BarAction}{\left\bracevert\phantom{A}\hspace{-9pt}\right.}

\newcommand{\Sing}{w}
\newcommand{\SingBar}{\overbarStraight{\Sing}}


\newcommand{\BrSep}[2]{\langle#1\rangle_{#2}}
%\newcommand{\dEmb}[1]{\dlfloor#1\drfloor}
\newcommand{\Emb}[2]{\llfloor#1\rrfloor_{#2}}
\newcommand{\im}{\textnormal{im}\,}
%\newcommand{\InvEmb}[2]{\llceil#1\rrceil^{#2}}
\newcommand{\InvEmb}[2]{\overhat{#1}}
\newcommand{\dInvEmb}[2]{\dlceil#1\drceil^{#2}}
\newcommand{\Kauf}[1]{\langle#1\rangle}
\newcommand{\cheque}{{\scaleobj{0.85}{\vee}}}

\newcommand{\SpecialPattern}{\mathsf{SP}}
\newcommand{\SpecialDiagram}{\mathsf{SD}}
\newcommand{\SpecialPatternBar}{\overbarStraight{\mathsf{SP}}}
\newcommand{\SpecialDiagramBar}{\overbarStraight{\mathsf{SD}}}


%\newcommand{\embed}{\iota}
\newcommand{\Gram}{\mathscr{G}}
\newcommand{\Uqsltwo}{{\mathsf{U}_q}}
\newcommand{\UqsltwoBar}{{\smash{\overbarStraight{\mathsf{U}}_q}}}
\newcommand{\Uqinvsltwo}{{\mathsf{U}^-_q}}
\newcommand{\UqsltwoPow}[1]{{\mathsf{U}^{\otimes #1}_q}}
\newcommand{\UqsltwoBarPow}[1]{{\smash{\overbarStraight{\mathsf{U}}}^{\otimes #1}_q}}

\newcommand{\EGen}{E}
\newcommand{\FGen}{F}
\newcommand{\KGen}{K}
\newcommand{\AntiEGen}{\smash{\overbarcal{\EGen}}}
\newcommand{\AntiFGen}{\smash{\overbarcal{\FGen}}}
\newcommand{\AntiKGen}{\smash{\overbarcal{\KGen}}}

\newcommand{\PlusEGen}{\EGen_+}
\newcommand{\PlusFGen}{\FGen_+}
\newcommand{\PlusKGen}{\KGen_+}
\newcommand{\MinusEGen}{\EGen_-}
\newcommand{\MinusFGen}{\FGen_-}
\newcommand{\MinusKGen}{\KGen_-}
\newcommand{\PlusMinusEGen}{\EGen_\pm}
\newcommand{\PlusMinusFGen}{\FGen_\pm}
\newcommand{\PlusMinusKGen}{\KGen_\pm}
\newcommand{\MinusPlusEGen}{\EGen_\mp}
\newcommand{\MinusPlusFGen}{\FGen_\mp}
\newcommand{\MinusPlusKGen}{\KGen_\mp}
\newcommand{\AntiPlusEGen}{\AntiEGen_+}
\newcommand{\AntiPlusFGen}{\AntiFGen_+}
\newcommand{\AntiPlusKGen}{\AntiKGen_+}
\newcommand{\AntiMinusEGen}{\AntiEGen_-}
\newcommand{\AntiMinusFGen}{\AntiFGen_-}
\newcommand{\AntiMinusKGen}{\AntiKGen_-}
\newcommand{\AntiPlusMinusEGen}{\AntiEGen_\pm}
\newcommand{\AntiPlusMinusFGen}{\AntiFGen_\pm}
\newcommand{\AntiPlusMinusKGen}{\AntiKGen_\pm}
\newcommand{\AntiMinusPlusEGen}{\AntiEGen_\mp}
\newcommand{\AntiMinusPlusFGen}{\AntiFGen_\mp}
\newcommand{\AntiMinusPlusKGen}{\AntiKGen_\mp}

\newcommand{\PlusUqSLTwo}{\mathsf{U}_{q+}}
\newcommand{\MinusUqSLTwo}{\mathsf{U}_{q-}}
\newcommand{\PlusMinusUqSLTwo}{\mathsf{U}_{q\pm}}
\newcommand{\MinusPlusUqSLTwo}{\mathsf{U}_{q\mp}}
\newcommand{\AntiPlusUqSLTwo}{\smash{\overbarStraight{\mathsf{U}}}_{q+}}
\newcommand{\AntiMinusUqSLTwo}{\smash{\overbarStraight{\mathsf{U}}}_{q-}}
\newcommand{\AntiPlusMinusUqSLTwo}{\smash{\overbarStraight{\mathsf{U}}}_{q\pm}}
\newcommand{\AntiMinusPlusUqSLTwo}{\smash{\overbarStraight{\mathsf{U}}}_{q\mp}}


\newcommand{\Usltwo}{\mathsf{U}}
\newcommand{\UqsltwoMod}{\Uqsltwo\textnormal{-Mod}_1}
\newcommand{\UsltwoMod}{\mathsf{U}\textnormal{-Mod}}
\newcommand{\FundBasis}{\varepsilon}
\newcommand{\FundBasisBar}{\overbarcal{\FundBasis}}
\newcommand{\Basis}{e}
\newcommand{\BasisBar}{\overbarStraight{\Basis}}
\newcommand{\np}{d}
\newcommand{\npp}{M}
\newcommand{\OneVec}[1]{\vec{#1}}
\newcommand{\LongOneVec}[1]{\overrightarrow{#1}}
%\newcommand{\SubOneVec}[1]{#1}
%\newcommand{\n}{{n}}%do not use!
\newcommand{\Summed}{n}
%\newcommand{\Defect}{u}%{t}%{\ss}%{\textit{\v{s}}}%{\cdprime}%{d}
\newcommand{\ExtraDefect}{v}
\newcommand{\sIndex}{s}
%\newcommand{\sIndexMax}{t}%do not use t here!?
%\newcommand{\s}{s}%do not use!
\newcommand{\HWsp}{\mathsf{H}}
\newcommand{\HWspBar}{\overbarStraight{\HWsp}}
%\newcommand{\HWspPerp}{\HWsp\superscr{\perp}}


\newcommand{\Ksp}{\mathsf{V}}
\newcommand{\KspBar}{\overbarStraight{\Ksp}}
\newcommand{\DefectSet}{\mathsf{E}}
\newcommand{\multii}{\varsigma}
\newcommand{\multiii}{\varpi}
\newcommand{\nprime}{m}

%\newcommand{\defect}[1]{\mathrm{def} \, #1}
\newcommand{\defect}[1]{\mathrm{def}_#1}



%\newcommand{\LeftUqAct}{\smash{\superscr{\Uqsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}}} \;}
%\newcommand{\RightUqAct}{\smash{\; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, \superscr{\,\Uqsltwo}}}
%\newcommand{\LeftUqBarAct}{\smash{\superscr{\UqsltwoBar\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}}} \;}
%\newcommand{\RightUqBarAct}{\smash{\; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, \superscr{\,\UqsltwoBar}}}
%\newcommand{\LeftUqUqBarAct}{\smash{\superscr{\Uqsltwo, \UqsltwoBar\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}}} \;}
%\newcommand{\RightUqUqBarAct}{\smash{\; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, \superscr{\,\Uqsltwo, \UqsltwoBar}}}


\newcommand{\VecSp}{\mathsf{V}}
\newcommand{\VecSpBar}{\overbarStraight{\VecSp}}
\newcommand{\VecSpInv}{\VecSp^-}

%\newcommand{\SpinChain}{\LeftUqAct \VecSp_\multii}
%\newcommand{\SpinChainBar}{\VecSpBar_\multii \RightUqAct}
%
%\newcommand{\SpinChainB}{\LeftUqUqBarAct \VecSp_\multii}
%\newcommand{\SpinChainBBar}{\VecSpBar_\multii \RightUqUqBarAct}

%\newcommand{\SpinChain}{\smash{{}\superscr{\Uqsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\SpinChain}{\mathsf{M}}
%\newcommand{\SpinChainBar}{\overbarStraight{\SpinChain}}
%\newcommand{\SpinChainBar}{\smash{{}\superscr{\UqsltwoBar\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSpBar}}
%\newcommand{\SpinChainInv}{\smash{{}\superscr{\Uqinvsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}^-}
%\newcommand{\SpinChainRegRight}{\smash{{}\superscr{\Uqsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSpBar}}
%\newcommand{\SpinChainRegTwistLeft}{\smash{{}\superscr{\Uqsltwo, \UqsltwoBar\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\SpinChainRegTwistRight}{\VecSpBar \RightUqAct}

%\newcommand{\SpinChainClass}{\smash{{}\superscr{\Usltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\SpinChainClassTL}{\smash{{}\subscr{\TL_\multii(-2)\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\SpinChainClassTL}{\smash{{}\subscr{\TL\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\BiSpinChainClass}{\smash{{}\superscr{\TL_\multii(-2) \otimes \Usltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\BiSpinChainClass}{\smash{{}\subscr{\TL_\multii(-2)}\superscr{\Usltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\BiSpinChainClass}{\smash{{}\subscr{\TL}\superscr{\Usltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}

%\newcommand{\SpinChainTL}{\smash{{}\superscr{\TL_\multii(\nu)\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\SpinChainTL}{\smash{{}\subscr{\TL_\multii(\nu)\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\SpinChainTL}{\smash{{}\subscr{\TL\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}

%\newcommand{\BiSpinChain}{\smash{{}\superscr{\TL_\multii(\nu) \otimes \Uqsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\BiSpinChain}{\smash{{}\subscr{\TL_\multii(\nu)}\superscr{\Uqsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}
%\newcommand{\BiSpinChain}{\smash{{}\subscr{\TL\,}\superscr{\Uqsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}}

\newcommand{\WdInv}{\smash{{}\superscr{\Uqinvsltwo\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; \VecSp}^-}

%\newcommand{\LeftTLAct}{\smash{{}\subscr{\TL\,} \scalebox{1}{\rotatebox[origin=c]{-90}{$\circlearrowright$}} \; }}
%\newcommand{\RightTLAct}{\smash{\; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, {}\subscr{\TL\,}}}


%\newcommand{\RightBothact}{\smash{\; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, {}\subscr{\TL\,}\superscr{\Uqsltwo\,}}}
%%\newcommand{\RightBothactClass}{\smash{\; \scalebox{1}{\rotatebox[origin=c]{90}{$\circlearrowleft$}} \, {}\subscr{\TL\,}\superscr{\Usltwo\,}}}

\newcommand{\HatBrep}{\smash{{\rm B}}}%this is not used?!?!?!?!?
\newcommand{\Brep}{{\mathscr{B}}}
\newcommand{\Trep}{{\mathscr{I}}}

\newcommand{\TrepBar}{\overbarcalcal{\Trep}}


\newcommand\und[1]{{\underset{\vspace{1pt} \scaleobj{1.4}{\check{}}}{#1}}}
\newcommand{\fds}{{\underset{\vspace{1pt} \scaleobj{1.4}{\check{}}}{\multii}}}
\newcommand{\lds}{{\hat{\multii}}}
\newcommand{\flds}{{\underset{\vspace{1pt} \scaleobj{1.4}{\check{}}}{\hat{\multii}}}}
\newcommand\munderbar[1]{\underaccent{\bar}{#1}}

\newcommand{\Srep}{\Brep}
\newcommand{\Rrep}{{\mathscr{C}}}

\newcommand{\HatPrep}{\smash{{\rm P}}}
\newcommand{\Prep}{{\rm P}}
%\newcommand{\hwvec}[2]{\smash{\tau^{#1}_{#2}}}
\newcommand{\HWvec}{u}%{\tau}
\newcommand{\HWvecBar}{\overbarcal{\HWvec}}


\newcommand{\HWvecMap}{\eta}
\newcommand{\HWvecMapBar}{\overbarcal{\eta}}



\newcommand{\super}[1]{^{\scaleobj{0.85}{(#1)}}}
\newcommand{\sub}[1]{_{\scaleobj{0.85}{(#1)}}}
\newcommand{\superscr}[1]{^{\scaleobj{0.85}{#1}}}
\newcommand{\subscr}[1]{_{\scaleobj{0.85}{#1}}}



\newcommand{\LSBiFormBar}[2]{(#1 \BarAction #2)}
%%\newcommand{\LSBiForm}[2]{(#1 \, , #2)}
%%\newcommand{\LSBiForm}[2]{\langle#1  \, , #2\rangle}
%\newcommand{\LSBiForm}[2]{\big( \hspace*{-1mm}| #1 , #2 |\hspace*{-1mm}\big) }
\newcommand{\LSBiForm}[2]{\boldsymbol{(}#1 \, , #2\boldsymbol{)}}


%\newcommand{\SPBiForm}[2]{\left(#1 , #2\right)}

%\newcommand{\SPBiFormNew}[2]{\big(#1 \,|\, #2 \big)}
%\newcommand{\SPBiFormNew}[2]{\left(#1 \,|\, #2 \right)}
%\newcommand{\SPBiFormNew}[2]{(#1 \,|\, #2)}


\newcommand{\SPBiForm}[2]{(#1 \,|\, #2)}
\newcommand{\SPBiFormBig}[2]{\big(#1 \,\big|\, #2 \big)}

%\global\long\def\Lpar{(\hspace*{-1mm}(}
%\global\long\def\Rpar{)\hspace*{-1mm})}

%\newcommand{\SPBiFormNewInv}[2]{\big\langle#1 \,|\, #2 \big\rangle}
%\newcommand{\SPBiFormNewInv}[2]{\big( \hspace*{-1mm}| #1 \,|\, #2 |\hspace*{-1mm}\big) }
\newcommand{\SPBiFormNewInv}[2]{\big( \hspace*{-1mm}| #1 \,,\, #2 |\hspace*{-1mm}\big) }
\newcommand{\SPBiFormInv}[2]{( \hspace*{-.85mm} \raisebox{.75pt}{\scaleobj{.80}{|}} #1 \,|\, #2 \raisebox{.75pt}{\scaleobj{.80}{|}}\hspace*{-.90mm})}
\newcommand{\SPBiFormBigInv}[2]{\big( \hspace*{-1mm}| #1 \,\big|\, #2 |\hspace*{-1mm}\big)}

%\newcommand{\Embedded}[3]{#1 \;}
%\newcommand{\Embedded}[3]{#1 \BarAction} 
%\newcommand{\Embedded}[3]{\left\llbracket #1 \right\rrbracket_{#2}^{#3}}
%\newcommand{\Embedded}[3]{\left\langle #1 \right\rangle_{#2}^{#3}}
\newcommand{\Dim}{D}
\newcommand{\Switch}{\chi}
%\newcommand{\projection}{\pi}
%\newcommand{\projectionhat}{\overhat{\projection}}
\newcommand{\WJProj}{P}%{\mathscr{P}}
\newcommand{\WJproj}{\WJProj}
\newcommand{\WJProjHat}{\overhat{\WJProj}}
\newcommand{\WJEmb}{I}
%\newcommand{\WalkMultii}{\varrho} don't use
\newcommand{\Rmatrix}{R}
\newcommand{\Rtrans}{r}
\newcommand{\cmap}{c}


%\newcommand{\LinkEmb}{\mathfrak{E}}
%\newcommand{\LinkEmb}{\WJEmb}


\newcommand{\one}{\mathbf{1} \hspace*{-.25em} \textnormal{l}}
%\newcommand{\one}{\mathtt{1}}

\newcommand{\antipode}{S}

\newcommand{\id}{\textnormal{id}}
\global\long\def\Projection{\mathfrak{P}}
\global\long\def\Projectionhat{\smash{\overhat{\Projection}}}
\global\long\def\Embedding{\mathfrak{I}}

\global\long\def\ProjectionBar{\overbarStraight{\Projection}}
\global\long\def\ProjectionhatBar{\smash{\overhat{\ProjectionBar}}}
\global\long\def\EmbeddingBar{\overbarStraight{\Embedding}}

\global\long\def\EmbeddingInv{\Embedding^-}


\newcommand{\hcrossing}{\;\vcenter{\hbox{\includegraphics[scale=0.275]{e-hcrossing.pdf}}}\;}
\newcommand{\ProjBox}{\;\vcenter{\hbox{\includegraphics[scale=0.275]{e-ProjBox.pdf}}}\;}
\global\long\def\SolSpCov{\mathsf{Sol}}
\global\long\def\SolSpLim{\mathsf{Lim}}

\newcommand{\const}{\mathrm{const.}}

%horizontal strikethrough
\newsavebox\CBox
\newcommand\hcancel[2][0.5pt]{%
  \ifmmode\sbox\CBox{$#2$}\else\sbox\CBox{#2}\fi%
  \makebox[0pt][l]{\usebox\CBox}%  
  \rule[0.5\ht\CBox-#1/2]{\wd\CBox}{#1}}
  
\global\long\def\qbin#1#2{\left[\begin{array}{c}
	#1\\
	#2 
	\end{array}\right]}
 

\newcommand{\defects}{%
 \,  \raisebox{-.4ex}{%
    \scalebox{1.2}{%
      \rotatebox[origin=c]{270}{$\exists$}%
    }%
  }%
}

\newcommand{\defectsBar}{%
 \,  \raisebox{-.4ex}{%
    \scalebox{1.2}{%
      \rotatebox[origin=c]{90}{$\exists$}%
    }%
  }%
}

%\newcommand{\defectsBar}{\rotatebox[origin=c]{270}{\defects}}


\newcommand{\defectsVal}{%
 \,  \raisebox{.4ex}{%
    \scalebox{1.1}{%
      \rotatebox[origin=c]{0}{$\mathbin{\stackanchor[-8.5pt]{\vee}{\perp}}$}%
    }%
  }%
}


\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}

\newcommand{\KWleq}{\stackrel{\scriptscriptstyle{()}}{\scriptstyle{\longleftarrow}}}
\newcommand{\KWgeq}{\stackrel{\scriptscriptstyle{()}}{\scriptstyle{\longrightarrow}}}

\newcommand{\DPle}{\prec} 
\newcommand{\DPleq}{\preceq} % partial order of DPs
\newcommand{\DPgeq}{\succeq} % partial order of DPs
\newcommand{\wedgeat}[1]{\lozenge_#1} % wedges of DPs
\newcommand{\upwedgeat}[1]{\wedge^#1}
\newcommand{\downwedgeat}[1]{\vee_#1}
\newcommand{\wedgelift}[1]{\uparrow \wedgeat{#1}} % wedge-lifting operation
\newcommand{\removewedge}[1]{\setminus \wedgeat{#1}}
\newcommand{\removeupwedge}[1]{\setminus \upwedgeat{#1}}
\newcommand{\removedownwedge}[1]{\setminus \downwedgeat{#1}}
\newcommand{\removeparen}[1]{\setminus \wedgeat{#1}}
\newcommand{\slopeat}[1]{\times_#1} % slope
\newcommand{\opar}{\rm{\url{(}}} % parenthesis notations have syntax {()()()}
\newcommand{\cpar}{\rm{\url{)}}}

\definecolor{amber}{rgb}{1.0, 0.75, 0.0}
\newcommand{\amber}{\textcolor{amber}}

\newcommand{\eve}{\textcolor{pink}}
\newcommand{\blue}{\textcolor{blue}}
%\newcommand{\blue}{\textcolor{SkyBlue}}

\newcommand{\red}{\textcolor{red}}
\newcommand{\Green}{\textcolor{green}}
\newcommand{\pink}{\textcolor{pink}}
\newcommand{\cyan}{\textcolor{cyan}}
\newcommand{\orange}{\textcolor{BurntOrange}}
\newcommand{\green}{\textcolor{JungleGreen}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}


\newcommand{\CCprojector}{\pi}
\newcommand{\CChatprojector}{\overhat{\CCprojector}}
\newcommand{\CCembedor}{\iota}

\newcommand{\CCprojectorBar}{\overbarcal{\CCprojector}}
\newcommand{\CChatprojectorBar}{\overhat{\CCprojectorBar}}
\newcommand{\CCembedorBar}{\overbarcal{\CCembedor}}

\newcommand{\CCembedorinv}{\CCembedor^-}



\newcommand{\CCunprojector}{\psi}
\newcommand{\CChatunprojector}{\overhat{\CCunprojector}}


\newcommand{\CCunprojectorBar}{\overbarcal{\CCunprojector}}
\newcommand{\CChatunprojectorBar}{\overhat{\CCunprojectorBar}}

%\newcommand{\CCprojector}[2]{\pi\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}
%\newcommand{\CChatprojector}[2]{\overhat{\pi}\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}
%\newcommand{\CCembedor}[2]{\iota\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}

%\newcommand{\CCprojectorBar}[2]{\overbarcal{\pi}\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}
%\newcommand{\CChatprojectorBar}[2]{\overhat{\overbarcal{\pi}}\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}
%\newcommand{\CCembedorBar}[2]{\overbarcal{\iota}\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}

%\newcommand{\CCembedorinv}[2]{(\iota^-)\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}

%\newcommand{\CCunprojector}[2]{\psi\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}
%\newcommand{\CChatunprojector}[2]{\overhat{\CCunprojector}\ifthenelse{\equal{#1}{}}{}{\super{#1}}\ifthenelse{\equal{#2}{}}{}{\sub{#2}}}


\newcommand{\isom}{\;\cong\;}

\newcommand{\LeftRegRep}{\rho}
\newcommand{\RightRegRep}{\overbarcal{\rho}}
\newcommand{\LeftTwistRep}{\tau}
\newcommand{\RightTwistRep}{\overbarcal{\tau}}



==> preamble.tex <==
\setlength{\paperheight}{11in}

\voffset=0.2in
\hoffset=-0.175in
\textheight=9.5in

\usepackage{array}
\usepackage{scalerel}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{stmaryrd}
\usepackage{amsthm}
\usepackage{graphicx} 
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{subeqnarray}
\usepackage[all]{xy}
\usepackage{accents}
\usepackage{subfigure}


\usepackage[pdftex, bookmarks, colorlinks=true, plainpages = false, citecolor = red, urlcolor = black, filecolor = blue]{hyperref}
\usepackage[usenames,dvipsnames]{color}
\usepackage[shortlabels]{enumitem}
\setenumerate{listparindent=\parindent}


\usepackage[titletoc]{appendix}
\renewcommand\appendixtocname{Appendix}
\renewcommand\appendixname{Appendix}
\renewcommand\appendixpagename{\centering \normalsize APPENDICES}

\newcommand{\itemcolor}[1]{
  \renewcommand{\makelabel}[1]{\color{#1}\hfil ##1}}

%This package has been added compared to the WJA papers.
\usepackage{stackengine}
\stackMath


\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * mathb
      <10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
\DeclareMathSymbol{\curvearrowright}{3}{mathb}{'361}

\usepackage{calligra}
\usepackage{tikz-cd}
\usepackage{thm-restate}
\DeclareMathAlphabet{\mathcalligra}{T1}{calligra}{m}{n}
\DeclareFontShape{T1}{calligra}{m}{n}{<->s*[2.2]callig15}{}

\def\dlceil{\left\lceil\kern-4.75pt\left\lceil}
\def\drceil{\right\rceil\kern-4.75pt\right\rceil}

\usepackage{etoolbox}
\patchcmd{\appendices}{\quad}{. }{}{}

\input{QSchurWeyl_macros.tex} %macro file is here


\theoremstyle{plain}
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section} % important bit
\newtheorem{prop}[theorem]{Proposition}
\numberwithin{prop}{section} % important bit
\newtheorem{cor}[theorem]{Corollary}
\numberwithin{cor}{section} % important bit
\newtheorem{lem}[theorem]{Lemma}
\numberwithin{lem}{section} % important bit
\newtheorem{conj}[theorem]{Conjecture}
\numberwithin{conj}{section} % important bit

%\theoremstyle{definition}
%\newtheorem{defn}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{condition}[theorem]{Condition}
%\newtheorem{example}[theorem]{Example} 
%\numberwithin{example}{section}
\newtheorem{quest}[theorem]{Question}
\numberwithin{quest}{section} % important bit

\newtheorem{claim}[theorem]{Claim}
\newtheorem{InductAssump}[theorem]{Induction Hypothesis}
\numberwithin{InductAssump}{section} % important bit
\newtheorem{comment}{Comment}
\numberwithin{comment}{section}

\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\numberwithin{remark}{section} % important bit
\newtheorem{recipe}[theorem]{Recipe}
\numberwithin{recipe}{section} % important bit
\newtheorem{defn}[theorem]{Definition}
\numberwithin{defn}{section} % important bit
\newtheorem{example}[theorem]{Example} 
\numberwithin{example}{section} % important bit


\makeatletter
\newenvironment{subtheorem}[1]{%
  \def\subtheoremcounter{#1}%
  \refstepcounter{#1}%
  \protected@edef\theparentnumber{\csname the#1\endcsname}%
  \setcounter{parentnumber}{\value{#1}}%
  \setcounter{#1}{0}%
  \expandafter\def\csname the#1\endcsname{\theparentnumber.\Alph{#1}}%
  \ignorespaces
}{%
  \setcounter{\subtheoremcounter}{\value{parentnumber}}%
  \ignorespacesafterend
}
\makeatother
\newcounter{parentnumber}


% Allows typesetting large summation/product indices without excessive blank space to the left or right of the sum/product.  Macros from http://www.tug.org/TUGboat/Articles/tb22-4/tb72perlS.pdf, p. 351.
%Example:  \[X = \sum_{\mathclap{1\le i\le j\le n}} X_{ij}\]
%Macros
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{%
\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{%
\rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{%
\clap{$\mathsurround=0pt#1{#2}$}}

%this creates the "backwared" \vec arrow
\makeatletter
\DeclareRobustCommand{\cev}[1]{%
  \mathpalette\do@cev{#1}%
}
\newcommand{\do@cev}[2]{%
  \fix@cev{#1}{+}%
  \reflectbox{$\m@th#1\vec{\reflectbox{$\fix@cev{#1}{-}\m@th#1#2\fix@cev{#1}{+}$}}$}%
  \fix@cev{#1}{-}%
}
\newcommand{\fix@cev}[2]{%
  \ifx#1\displaystyle
    \mkern#23mu
  \else
    \ifx#1\textstyle
      \mkern#23mu
    \else
      \ifx#1\scriptstyle
        \mkern#22mu
      \else
        \mkern#22mu
      \fi
    \fi
  \fi
}

%number equations by section
\numberwithin{equation}{section}

%number figures by section
\numberwithin{figure}{section}


\renewcommand{\thesection}{\arabic{section}} 

\makeatother

\allowdisplaybreaks


